Cost Sharing in Two-Sided Markets

Motivated by the emergence of popular service-based two-sided markets where sellers can serve multiple buyers at the same time, we formulate and study the {\em two-sided cost sharing} problem. In two-sided cost sharing, sellers incur different costs for serving different subsets of buyers and buyers have different values for being served by different sellers. Both buyers and sellers are self-interested agents whose values and costs are private information. We study the problem from the perspective of an intermediary platform that matches buyers to sellers and assigns prices and wages in an effort to maximize welfare (i.e., buyer values minus seller costs) subject to budget-balance in an incentive compatible manner. In our markets of interest, agents trade the (often same) services multiple times. Moreover, the value and cost for the same service differs based on the context (e.g., location, urgency, weather conditions, etc). In this framework, we design mechanisms that are efficient, ex-ante budget-balanced, ex-ante individually rational, dominant strategy incentive compatible, and ex-ante in the core (a natural generalization of the core that we define here).

==> tex/macros.tex <==
\usepackage[T1]{fontenc}
\usepackage[utf8]{inputenc}
\usepackage{authblk}
\usepackage{fullpage}
\usepackage{amstext,amssymb}
\usepackage{amsmath}
\usepackage{amsthm}
%\usepackage[parfill]{parskip}
\usepackage{comment}
\usepackage{xcolor}
\usepackage{bbm}
\usepackage{mathtools}
\linespread{1}

\usepackage[margin=0.99in]{geometry}
%\usepackage[top=1.1in, bottom=1.2in, left=1.11in, right=1.11in]{geometry}
\usepackage{ifthen}
\usepackage{algpseudocode,algorithm,algorithmicx}
\newcommand*\DNA{\textsc{dna}}
\newcommand*\Let[2]{\State #1 $\gets$ #2}
\algrenewcommand\algorithmicrequire{\textbf{Precondition:}}
\algrenewcommand\algorithmicensure{\textbf{Postcondition:}}
\usepackage{graphicx,color}
\usepackage{fancybox}
\usepackage{lipsum}
\usepackage{array,float}
\usepackage{url}
%\begingroup
%    \makeatletter
%    \@for\theoremstyle:=definition,remark,plain\do{%
%        \expandafter\g@addto@macro\csname th@\theoremstyle\endcsname{%
%            \addtolength\thm@preskip\parskip
%            }%
%        }
%\endgroup
\usepackage{mathrsfs}
\usepackage{dsfont}
\definecolor{cornellred}{rgb}{0.7, 0.11, 0.11}
\definecolor{dgreen}{rgb}{0.0, 0.5, 0.0}
\definecolor{ballblue}{rgb}{0.13, 0.67, 0.8}
\definecolor{royalblue(web)}{rgb}{0.25, 0.41, 0.88}
\definecolor{bleudefrance}{rgb}{0.19, 0.55, 0.91}
\definecolor{royalazure}{rgb}{0.0, 0.22, 0.66}
\usepackage{hyperref}
\hypersetup{
    colorlinks = true,
    linkcolor=cornellred,
    citecolor=royalazure,
    linkbordercolor = {white}
}
\usepackage{cleveref}
%\usepackage{pstricks,pst-tree,pst-node}
\usepackage[shortlabels]{enumitem}


\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem*{lemma*}{Lemma}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{observation}{Observation}
\theoremstyle{definition}
\newtheorem{definition}{Definition}[section]
\theoremstyle{definition}
\newenvironment{example}[1][Example]{\begin{trivlist}
\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}
\newenvironment{remark}[1][Remark]{\begin{trivlist}
\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}

%\renewcommand{\qed}{\nobreak \ifvmode \relax \else
%      \ifdim\lastskip<1.5em \hskip-\lastskip
%      \hskip1.5em plus0em minus0.5em \fi \nobreak
%      \vrule height0.75em width0.5em depth0.25em\fi}

\usepackage{accents}
\usepackage[authoryear,round]{natbib}

%\newcommand{\ubar}[1]{\underaccent{\bar}{#1}}
%\newcommand{\reals}{\mathbb{R}}
\newcommand*{\R}{\mathbb{R}}





\DeclareMathOperator{\argmax}{argmax}
\DeclareMathOperator{\argmin}{argmin}
\DeclareMathOperator{\OPT}{OPT}
\DeclarePairedDelimiter{\norm}{\lVert}{\rVert}
\DeclarePairedDelimiter{\card}{\lvert}{\rvert}
\DeclarePairedDelimiter{\abs}{\lvert}{\rvert}
\providecommand{\given}{}
\DeclarePairedDelimiterX{\set}[1]\{\}{\renewcommand\given{\nonscript\:\delimsize\vert\nonscript\:\mathopen{}}#1}
\let\Pr\relax
\DeclarePairedDelimiterXPP{\Pr}[1]{\mathbb{P}}[]{}{\renewcommand\given{\nonscript\:\delimsize\vert\nonscript\:\mathopen{}}#1}
\DeclarePairedDelimiterXPP{\Ex}[1]{\mathbb{E}}[]{}{\renewcommand\given{\nonscript\:\delimsize\vert\nonscript\:\mathopen{}}#1}
\DeclarePairedDelimiter{\dotp}{\langle}{\rangle}



%################# Macros for this paper ########################
\newcommand{\eps}{\epsilon}
\newcommand{\as}[1]{{\color{red} {(\sf Amin:} {\sl{#1}}     {\sf )}}}
\newcommand{\ali}[1]{{\color{blue} {(\sf Ali:} {\sl{#1}}     {\sf )}}}
\newcommand{\rn}[1]{{\color{red} {(\sf Rad:} {\sl{#1}}     {\sf )}}}
\newcommand{\nal}[1]{{\color{cyan} {(\sf Nima:} {\sl{#1}}     {\sf )}}}

\newcommand{\sep}{\gamma}
\newcommand{\soft}{\mathcal{S}}
\newcommand{\X}{\mathcal{X}}
\newcommand{\Y}{\mathcal{Y}}
\newcommand{\Exv}[2]{\mathbb{E}_{#1}\left[#2\right]}
\newcommand{\V}{\mathcal{V}}
\newcommand{\T}{\tau}
\newcommand{\vr}{\vec{r}}
\newcommand{\Z}{\mathcal{Z}}
\newcommand{\Sm}{\mathscr{S}}
\newcommand{\La}{\mathscr{L}}
\newcommand{\Po}{\mathcal{P}}
\newcommand{\1}[1]{\mathds{1}\left[#1\right]}


